Majority Voting for Code Generation

We investigate Functional Majority Voting (FMV), a method based on functional consensus for code generation with Large Language Models, which identifies a representative solution from multiple generations using their runtime execution signatures on test inputs. We find that FMV is an effective test-time inference strategy, substantially boosting performance on LiveCodeBench without a large compute overhead. Furthermore, we extend the utility of functional consensus and apply it as an aggregation strategy for label-free Test-Time Reinforcement Learning. We demonstrate that this increases pass@1 on holdout tasks, but find no evidence of self-improvement beyond the base model's performance ceiling.

==> figs/barplot1.tex <==
\begin{tikzpicture}
    \begin{axis}[
        ybar,
        % --- 1. Dimensions & Fonts ---
        width=\linewidth,       % Fills the minipage
        height=5.5cm,           % Fixed height matches line plot
        tick label style={font=\small},
        label style={font=\small},
        legend style={font=\footnotesize},
        % --- 2. Spacing Fix ---
        ylabel near ticks,      % Pulls "Accuracy" closer
        bar width=8pt,
        enlarge x limits=0.2,
        symbolic x coords={4B-Instr, 30B-Instr, 4B-Think, 30B-Think},
        xtick=data,
        ylabel={Accuracy (\%)},
        ymin=25, ymax=70,
        ymajorgrids=true,
        grid style={dashed, gray!30},
        xticklabel style={rotate=0, align=center},
        legend style={
            at={(0.5,1.05)}, 
            anchor=south, 
            legend columns=-1,
            draw=none,
            /tikz/every even column/.append style={column sep=0.3cm}
        },
    ]
    % 1. Base Model
    \addplot+[teal!80!black, fill=teal!30, error bars/.cd, y dir=both, y explicit] 
        coordinates {
        (4B-Instr, 30.8) 
        (30B-Instr, 35.9) 
        (4B-Think, 37.7) 
        (30B-Think, 48.0)
        };
    \addlegendentry{Base}
    % 2. Semantic Voting
    \addplot+[orange!90!black, fill=orange!30] 
        coordinates {
        (4B-Instr, 34.8) 
        (30B-Instr, 42.7) 
        (4B-Think, 48.1) 
        (30B-Think, 59.0) 
        };
    \addlegendentry{Sem. Vote}
    % 3. GenCluster
    \addplot+[violet!90!black, fill=violet!30] 
        coordinates {
        (4B-Instr, 32.0) 
        (30B-Instr, 37.8) 
        (4B-Think, 52.7) 
        (30B-Think, 61.3) 
        };
    \addlegendentry{GenCluster}
    % 4. Joint-FMV
    \addplot+[blue!70!white, fill=blue!30, error bars/.cd, y dir=both, y explicit] 
        coordinates {
        (4B-Instr, 41.2)
        (30B-Instr, 49.6)
        (4B-Think, 51.9)
        (30B-Think, 64.8)
        };
    \addlegendentry{FMV (ours)}
    \end{axis}
\end{tikzpicture}

==> figs/lineplot1.tex <==
\begin{tikzpicture}
    \begin{axis}[
        % --- 1. Dimensions & Fonts ---
        width=\linewidth,       % Fills the minipage
        height=5.5cm,           % Fixed height for alignment
        tick label style={font=\small},
        label style={font=\small},
        legend style={font=\footnotesize},
        
        % --- 2. Spacing Fix ---
        ylabel near ticks,      % Pulls "Accuracy" closer to the numbers
        
        grid=major,
        grid style={dashed, gray!30},
        xlabel={Number of Completions ($N$)},
        ylabel={Accuracy (\%)},
        
        % Log Scale Setup
        xmode=log,
        log basis x={2},
        xtick={1, 2, 4, 8, 16, 32, 64},
        xticklabels={1, 2, 4, 8, 16, 32, 64},
        
        % Visual limits
        ymin=28, ymax=45,
        xmin=0, xmax=64,
        
        % Legend Setup
        legend style={
            at={(0.5,1.05)}, 
            anchor=south, 
            legend columns=-1,
            draw=none,
            /tikz/every even column/.append style={column sep=0.3cm}
        },
        tick align=outside,
        tick pos=left
    ]

    % --- 1. BASELINE (Teal - Matched to Bar Plot) ---
    % Upper Bound
    \addplot[name path=base_top, draw=none, forget plot] coordinates {
        (1, 30.5) (2, 30.5) (4, 30.5) (8, 30.5) (16, 30.5) (24, 30.5) (32, 30.5) (40, 30.5) (48, 30.5) (56, 30.5) (64, 30.5)
    };
    % Lower Bound
    \addplot[name path=base_bot, draw=none, forget plot] coordinates {
        (1, 30.5) (2, 30.5) (4, 30.5) (8, 30.5) (16, 30.5) (24, 30.5) (32, 30.5) (40, 30.5) (48, 30.5) (56, 30.5) (64, 30.5)
    };
    % Fill (Updated to teal!30)
    \addplot[teal!30, opacity=0.5, forget plot] fill between[of=base_top and base_bot];
    % Main Line (Updated to teal!80!black)
    \addplot[
        color=teal!80!black,
        mark=*,
        line width=1.5pt
    ] coordinates {
        (1, 30.5) (2, 30.5) (4, 30.5) (8, 30.5) (16, 30.5) (24, 30.5) (32, 30.5) (40, 30.5) (48, 30.5) (56, 30.5) (64, 30.5)
    };
    \addlegendentry{Baseline}

    % --- 2. SEMANTIC VOTING (Orange - Matched Opacity) ---
    \addplot[name path=sem_top, draw=none, forget plot] coordinates {
        (1, 30.5) (2, 32.2) (4, 33.5) (8, 34.3) (16, 34.8) (24, 35.3) (32, 34.6) (40, 35.8) (48, 33.8) (56, 35.3) (64, 34.4)
    };
    \addplot[name path=sem_bot, draw=none, forget plot] coordinates {
        (1, 30.5) (2, 28.8) (4, 30.2) (8, 30.7) (16, 31.8) (24, 32.5) (32, 31.4) (40, 32.6) (48, 31.6) (56, 32.5) (64, 33.6)
    };
    % Fill (Updated to !30)
    \addplot[orange!30, opacity=0.5, forget plot] fill between[of=sem_top and sem_bot];
    \addplot[
        color=orange!90!black,
        mark=triangle*,
        line width=1.5pt
    ] coordinates {
        (1, 30.5) (2, 30.0) (4, 31.9) (8, 32.5) (16, 33.3) (24, 33.9) (32, 33.0) (40, 34.2) (48, 32.7) (56, 33.9) (64, 34.0)
    };
    \addlegendentry{Semantic Voting}

    % --- 3. JOINT-FMV (Blue - Matched Opacity) ---
    \addplot[name path=fmv_top, draw=none, forget plot] coordinates {
        (1, 30.5) (2, 34.0) (4, 36.5) (8, 39.6) (16, 40.8) (24, 40.8) (32, 41.3) (40, 42.0) (48, 41.0) (56, 42.0) (64, 41.2)
    };
    \addplot[name path=fmv_bot, draw=none, forget plot] coordinates {
        (1, 30.5) (2, 30.8) (4, 33.5) (8, 36.8) (16, 38.6) (24, 38.0) (32, 39.9) (40, 40.8) (48, 40.0) (56, 40.8) (64, 40.4)
    };
    % Fill (Updated to !30)
    \addplot[blue!30, opacity=0.5, forget plot] fill between[of=fmv_top and fmv_bot];
    \addplot[
        color=blue!70!white,
        mark=square*,
        line width=1.5pt
    ] coordinates {
        (1, 30.5) (2, 32.4) (4, 35.0) (8, 38.2) (16, 39.7) (24, 39.4) (32, 40.6) (40, 41.4) (48, 40.5) (56, 41.4) (64, 40.8)
    };
    \addlegendentry{FMV (ours)}
    \end{axis}
\end{tikzpicture}

==> figs/scaling-N.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=0.6\linewidth,
            height=5.5cm,
            grid=major,
            grid style={dashed, gray!30},
            xlabel={Number of Completions ($N$)},
            ylabel={Accuracy (\%)},
            % Log Scale Setup
            xmode=log,
            log basis x={2},
            xtick={1, 2, 4, 8, 16, 32, 64},
            xticklabels={1, 2, 4, 8, 16, 32, 64},
            % Visual limits
            ymin=28, ymax=45,
            xmin=0, xmax=64,
            % Legend Setup
            legend style={
                at={(0.5,1.05)}, 
                anchor=south, 
                legend columns=-1,
                draw=none,
                /tikz/every even column/.append style={column sep=0.3cm}
            },
            tick align=outside,
            tick pos=left
        ]

        % --- 1. BASELINE (Gray) ---
        % Upper Bound (Invisible)
        \addplot[name path=base_top, draw=none, forget plot] coordinates {
            (1, 30.5) (2, 30.5) (4, 30.5) (8, 30.5) (16, 30.5) (24, 30.5) (32, 30.5) (40, 30.5) (48, 30.5) (56, 30.5) (64, 30.5)
        };
        % Lower Bound (Invisible)
        \addplot[name path=base_bot, draw=none, forget plot] coordinates {
            (1, 30.5) (2, 30.5) (4, 30.5) (8, 30.5) (16, 30.5) (24, 30.5) (32, 30.5) (40, 30.5) (48, 30.5) (56, 30.5) (64, 30.5)
        };
        % Fill
        \addplot[gray!20, opacity=0.5, forget plot] fill between[of=base_top and base_bot];
        % Main Line
        \addplot[
            color=gray,
            mark=*,
            line width=1.5pt
        ] coordinates {
            (1, 30.5) (2, 30.5) (4, 30.5) (8, 30.5) (16, 30.5) (24, 30.5) (32, 30.5) (40, 30.5) (48, 30.5) (56, 30.5) (64, 30.5)
        };
        \addlegendentry{Baseline}

        % --- 2. SEMANTIC VOTING (Orange) ---
        % Upper Bound
        \addplot[name path=sem_top, draw=none, forget plot] coordinates {
            (1, 30.5) (2, 32.2) (4, 33.5) (8, 34.3) (16, 34.8) (24, 35.3) (32, 34.6) (40, 35.8) (48, 33.8) (56, 35.3) (64, 34.4)
        };
        % Lower Bound
        \addplot[name path=sem_bot, draw=none, forget plot] coordinates {
            (1, 30.5) (2, 28.8) (4, 30.2) (8, 30.7) (16, 31.8) (24, 32.5) (32, 31.4) (40, 32.6) (48, 31.6) (56, 32.5) (64, 33.6)
        };
        % Fill
        \addplot[orange!20, opacity=0.5, forget plot] fill between[of=sem_top and sem_bot];
        % Main Line
        \addplot[
            color=orange!90!black,
            mark=triangle*,
            line width=1.5pt
        ] coordinates {
            (1, 30.5) (2, 30.0) (4, 31.9) (8, 32.5) (16, 33.3) (24, 33.9) (32, 33.0) (40, 34.2) (48, 32.7) (56, 33.9) (64, 34.0)
        };
        \addlegendentry{Semantic Voting}

        % --- 3. JOINT-FMV (Blue - Ours) ---
        % Upper Bound
        \addplot[name path=fmv_top, draw=none, forget plot] coordinates {
            (1, 30.5) (2, 34.0) (4, 36.5) (8, 39.6) (16, 40.8) (24, 40.8) (32, 41.3) (40, 42.0) (48, 41.0) (56, 42.0) (64, 41.2)
        };
        % Lower Bound
        \addplot[name path=fmv_bot, draw=none, forget plot] coordinates {
            (1, 30.5) (2, 30.8) (4, 33.5) (8, 36.8) (16, 38.6) (24, 38.0) (32, 39.9) (40, 40.8) (48, 40.0) (56, 40.8) (64, 40.4)
        };
        % Fill
        \addplot[blue!20, opacity=0.5, forget plot] fill between[of=fmv_top and fmv_bot];
        % Main Line
        \addplot[
            color=blue!70!white,
            mark=square*,
            line width=1.5pt
        ] coordinates {
            (1, 30.5) (2, 32.4) (4, 35.0) (8, 38.2) (16, 39.7) (24, 39.4) (32, 40.6) (40, 41.4) (48, 40.5) (56, 41.4) (64, 40.8)
        };
        \addlegendentry{FMV (ours)}
        \end{axis}
    \end{tikzpicture}
    \caption{Scaling of voting methods with rollout budget $N$ (log-scale). While Semantic Voting (Orange) yields marginal gains over the Baseline (Gray), FMV (Blue) scales efficiently, achieving over $40\%$ accuracy with as few as $N=32$ samples.}
    \label{fig:scaling-lines}
\end{figure}

==> figs/test-time-inference.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            bar width=8pt,
            enlarge x limits=0.2,
            % Define the models as x-coordinates
            symbolic x coords={4B-Instr, 30B-Instr, 4B-Think, 30B-Think},
            xtick=data,
            ylabel={Accuracy (\%)},
            ymin=25, ymax=70, % Adjusted ymax to fit the highest bar (64.8)
            ymajorgrids=true,
            grid style={dashed, gray!30},
            xticklabel style={rotate=0, align=center, font=\small},
            % Legend configuration
            legend style={
                at={(0.5,1.05)}, 
                anchor=south, 
                legend columns=-1,
                draw=none,
                font=\footnotesize,
                /tikz/every even column/.append style={column sep=0.3cm}
            },
            width=0.7\linewidth,
            height=5.5cm,
        ]
        
        % 1. Base Model (Gray)
        \addplot+[teal!80!black, fill=teal!30, error bars/.cd, y dir=both, y explicit] 
            coordinates {
            (4B-Instr, 30.8) % +=(0,3.2) -=(0,3.2)
            (30B-Instr, 35.9) %+=(0,3.7) -=(0,3.7)
            (4B-Think, 37.7) % +=(0,3.7) -=(0,3.7)
            (30B-Think, 48.0)%  +=(0,3.8) -=(0,3.8)
            };
        \addlegendentry{Base}

        % 2. Semantic Voting (Orange)
        \addplot+[orange!90!black, fill=orange!30] 
            coordinates {
            (4B-Instr, 34.8) 
            (30B-Instr, 42.7) 
            (4B-Think, 48.1) 
            (30B-Think, 59.0) 
            };
        \addlegendentry{Sem. Vote}

        % 3. GenCluster (Violet)
        \addplot+[violet!90!black, fill=violet!30] 
            coordinates {
            (4B-Instr, 32.0) 
            (30B-Instr, 37.8) 
            (4B-Think, 52.7) 
            (30B-Think, 61.3) 
            };
        \addlegendentry{GenCluster}
        
        % 4. Joint-FMV (Blue - Ours)
        \addplot+[blue!70!white, fill=blue!30, error bars/.cd, y dir=both, y explicit] 
            coordinates {
            (4B-Instr, 41.2)% +=(0,4.3) -=(0,4.3)
            (30B-Instr, 49.6)% +=(0,4.2) -=(0,4.2)
            (4B-Think, 51.9) %+=(0,4.3) -=(0,4.3)
            (30B-Think, 64.8)% +=(0,4.0) -=(0,4.0)
            };
        \addlegendentry{FMV (ours)}
        
        \end{axis}
    \end{tikzpicture}
    \caption{Test-time inference scaling on LCBv6 ($N=64$) across model families. Joint-FMV (Blue) consistently outperforms Semantic Voting (Orange) and Base performance (Teal), and performs on par with GenCluster (Violet).}
    \label{fig:multimodel-barchart}
\end{figure}
